Hybrid Spectral Denoising Transformer with Guided Attention

In this paper, we present a Hybrid Spectral Denoising Transformer (HSDT) for hyperspectral image denoising. Challenges in adapting transformer for HSI arise from the capabilities to tackle existing limitations of CNN-based methods in capturing the global and local spatial-spectral correlations while maintaining efficiency and flexibility. To address these issues, we introduce a hybrid approach that combines the advantages of both models with a Spatial-Spectral Separable Convolution (S3Conv), Guided Spectral Self-Attention (GSSA), and Self-Modulated Feed-Forward Network (SM-FFN). Our S3Conv works as a lightweight alternative to 3D convolution, which extracts more spatial-spectral correlated features while keeping the flexibility to tackle HSIs with an arbitrary number of bands. These features are then adaptively processed by GSSA which per-forms 3D self-attention across the spectral bands, guided by a set of learnable queries that encode the spectral signatures. This not only enriches our model with powerful capabilities for identifying global spectral correlations but also maintains linear complexity. Moreover, our SM-FFN proposes the self-modulation that intensifies the activations of more informative regions, which further strengthens the aggregated features. Extensive experiments are conducted on various datasets under both simulated and real-world noise, and it shows that our HSDT significantly outperforms the existing state-of-the-art methods while maintaining low computational overhead. Code is at https: //github.com/Zeqiang-Lai/HSDT.

==> figures/complex2.tex <==
\begin{figure*}
\captionsetup[subfigure]{labelformat=empty}
\begin{center}
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/noisy.png}
         \caption{Noisy}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/LRTV}
         \caption{LRTV \cite{he2015total}}
     \end{subfigure}
      \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/nmog}
         \caption{NMoG \cite{chen2017denoising}}
     \end{subfigure}
      \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/tdtv}
         \caption{TDTV \cite{wang2017hyperspectral}}
     \end{subfigure}
      \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/hsid_cnn}
         \caption{HSID-CNN \cite{yuan2018hyperspectral}}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/qrnn3d}
         \caption{QRNN3D \cite{wei20203}}
     \end{subfigure}
     \quad
      \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/gt}
         \caption{Ground Truth}
     \end{subfigure}
      \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/grunet}
         \caption{GRUNet \cite{lai2022deep}}
     \end{subfigure}
      \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/restormer_b31}
         \caption{Restormer \cite{zamir2022restormer}}
     \end{subfigure}
      \hfill
     \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/trq3d}
         \caption{TRQ3D \cite{pang2022trq3dnet}}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/trq3d}
         \caption{SST \cite{li2022spatial}}
     \end{subfigure}
     \hfill
      \begin{subfigure}[b]{0.15\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/simulated/lehavim_0910-1605_icvl_512_stripe/hsdt}
         \caption{HSDT-L(ours)}
     \end{subfigure}
     \end{center}
    \vspace{-6mm}
   \caption{Simulated complex noise removal results of synthetic color image on ICVL dataset. (\emph{stripe} case)}
   \label{fig:complex}
   \vspace{-2mm}
\end{figure*}

==> figures/gaussian2.tex <==
\begin{figure*}[ht]
\captionsetup[subfigure]{labelformat=empty}
    \begin{center}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/noisy}
          \caption{Noisy}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/llrt}
          \caption{LLRT \cite{chang2017hyper}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/kbr}
          \caption{KBR\cite{Qi2017Kronecker}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/wlrtr}
          \caption{WLRTR\cite{chang2020weighted}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/ngmeet}
          \caption{NGmeet\cite{he2019non}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/hsid_cnn}
          \caption{HSIDCNN\cite{yuan2018hyperspectral}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/qrnn3d}
          \caption{QRNN3D\cite{wei20203}}
      \end{subfigure}
      \quad 
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/gt}
          \caption{Ground Truth}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/t3sc}
          \caption{T3SC\cite{bodrito2021trainable}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/grunet}
          \caption{GRUNet\cite{lai2022deep}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/restormer_b31}
          \caption{Restormer\cite{zamir2022restormer}}
      \end{subfigure}
       \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/trq3d}
          \caption{TRQ3D\cite{pang2022trq3dnet}}
      \end{subfigure}
       \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/trq3d}
          \caption{SST\cite{li2022spatial}}
      \end{subfigure}
      \begin{subfigure}[b]{0.138\textwidth}
          \centering
          \includegraphics[width=\textwidth]{imgs/simulated/objects_0924-1650_icvl_512_50/hsdt_deep}
          \caption{HSDT-L(ours)}
      \end{subfigure}
	\end{center}
	\vspace{-5mm}
    \caption{Simulated Gaussian noise removal results of synthetic color image under noise level $\sigma=50$ on ICVL dataset.}
    \label{fig:gaussian}
    \vspace{-2mm}
 \end{figure*}

==> tables/ablation_components.tex <==




\begin{table*}[t]
   \begin{subtable}[h]{0.34\textwidth}
      \setlength{\tabcolsep}{0.162cm}
       \centering
       \small
       \begin{tabular}{l| l| l| l}
         \hline
      \rowcolor{graycolor} Model  & Params & PSNR & SAM \\
       \hline
       Conv3D & 0.43/0.58M & 41.62 & 0.052\\
       Sep3D \cite{dong2019deep}  & 0.37/0.53M & 41.44 & 0.054\\
       \hline
       S3Conv-Seq  & 0.26/0.42M & 41.58 & 0.052\\
       S3Conv  & 0.36/0.52M & \textbf{41.82} & \textbf{0.049} \\
       \hline
      \end{tabular}
      \caption{Different variants of our S3Conv in comparison with 3D convolution.  }
      \label{tab:ablation-s3conv}
   \end{subtable}
   \hfill
   \begin{subtable}[h]{0.3\textwidth}
   \setlength{\tabcolsep}{0.14cm}
       \centering
       \small
       \begin{tabular}{l | l | l | l}
         \hline
         \rowcolor{graycolor} Model & Params & PSNR & SAM \\
       \hline 
     QRU \cite{wei20203}  & 0.57M & 41.31 & 0.064\\
     SSA-2D \cite{li2022spatial} & 4.14M & 41.41 & 0.052\\
       GSSA & 0.51M & 41.80 & 0.050\\
       GSSA & 0.52M & \textbf{41.82} & \textbf{0.049}\\
       \hline
      \end{tabular}
 	\caption{Results of our GSSA and GSSA in comparison with other attention blocks.}
      \label{tab:ablation-ssa}
   \end{subtable}
   \hfill
    \begin{subtable}[h]{0.3\textwidth}
    \setlength{\tabcolsep}{0.15cm}
       \centering
       \small
       \begin{tabular}{l | l | l | l}
         \hline
    \rowcolor{graycolor} Model  & Params & PSNR & SAM \\
       \hline
       FFN & 0.49M & 41.67 & 0.050\\
       GDFN \cite{zamir2022restormer} & 0.49M &37.38 & 0.094\\
       \hline
       SM-Branch  & 0.45M &41.74 & 0.051\\
       SM-FFN  & 0.52M & \textbf{41.82} & \textbf{0.049} \\
       \hline
      \end{tabular}
      \caption{Comparison of the existing FFN with our SM-FFN and SM-Branch.  }
      \label{tab:ablation-ffn}
   \end{subtable} 
   \vspace{-2mm}
    \caption{Design choices. We compare each block by replacing it with others while keeping other parts the same as HSDT-M. As 2D spectral self-attention (SSA-2D) in \cite{li2022spatial} could not fit into our 3D architecture, we report the results of their own model. }
    \label{tab:temps}
    \vspace{-2mm}
\end{table*}
